Trex: Learning Execution Semantics from Micro-Traces for Binary Similarity

Detecting semantically similar functions -- a crucial analysis capability with broad real-world security usages including vulnerability detection, malware lineage, and forensics -- requires understanding function behaviors and intentions. This task is challenging as semantically similar functions can be implemented differently, run on different architectures, and compiled with diverse compiler optimizations or obfuscations. Most existing approaches match functions based on syntactic features without understanding the functions' execution semantics. We present Trex, a transfer-learning-based framework, to automate learning execution semantics explicitly from functions' micro-traces and transfer the learned knowledge to match semantically similar functions. Our key insight is that these traces can be used to teach an ML model the execution semantics of different sequences of instructions. We thus train the model to learn execution semantics from the functions' micro-traces, without any manual labeling effort. We then develop a novel neural architecture to learn execution semantics from micro-traces, and we finetune the pretrained model to match semantically similar functions. We evaluate Trex on 1,472,066 function binaries from 13 popular software projects. These functions are from different architectures and compiled with various optimizations and obfuscations. Trex outperforms the state-of-the-art systems by 7.8%, 7.2%, and 14.3% in cross-architecture, optimization, and obfuscation function matching, respectively. Ablation studies show that the pretraining significantly boosts the function matching performance, underscoring the importance of learning execution semantics.

==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}

\vspace{.1cm}
\noindent\textbf{Definition of pretraining and finetuning.}
A typical difference between pretraining and finetuning in NLP is pretraining is often self-/un-supervised while finetuning is supervised. 
Besides, pretraining is often believed responsible for heavy-lifting, with huge amount of training corpus and parameter updates. While in finetuning, the training process often does not significantly update the ``knowledge'' of the pretrained model. Instead, it is often light-weight with small extra layers and number of training epochs.
In general, pretraining learns task-agnostic general knowledge while finetuning learns for task-specific downstream tasks.

In the setting of this project, such distinction becomes not so obvious, as our finetuning task (function similarity) does not necessarily requires any labeling effort. Particularly, we can cheaply collect the same source code and compile into different architectures, optimizations, and obfuscations. Therefore, we believe our finetuning task can also be leveraged to learn general semantic representation of the code. By encouraging the model to produce similar embeddings for same functions with different transformations, we teach the model invariances of underlying code semantics.
We plan to explore this direction in the future work.

==> intro.bck.tex <==
\section{Introduction}
\label{sec:intro}


% - Finding similar code has many security applications. (give example that we are doing)\\
% - However, finding structural similarity is not enough. (explain why)\\
% - Thus, it is important to understand semantic similarity between different code fragments. \\
% - Semantics can be best inferred by code execution. \\
% - But it is often inefficient because there are many paths. --> introduce micro execution\\
% - The whole problem aggravates if it is in binary as even structure contains lot of noise\\
% - Thus, we present an ML model to establish semantic similarity.\\
% - We demonstrate its effectiveness in X and Y applications.\\
% There have been a significant amount of advances in program representation and consequently automated static analysis techniques, with the rise of machine learning being used for learning these program embeddings. 
% However, static program representation learning has some fundamental shortcomings. Firstly, in order to automate and scale static analysis, defining complex platform specific rules and heuristics is a time consuming process, especially if you're dealing with binaries compiled across different platforms, different protocols, etc. Moreover, using static analysis can often lead to modeling imprecise dependencies (e.g. non existent relationships) between variables whereas an execution may easily reveal these deeper relationships at runtime. 

% Learning effective code representations that captures code's functionality and intent is important but nontrivial. Unlike natural language, program code can be executed and its semantics are encoded in not only static instructions but also dynamic execution traces. 
% Therefore, we develop \sys, which aims to augment the representation learning of traditional static code with dynamic execution information, to learn program representations that closely reflects execution semantics. 

% Specifically, we apply the self-supervised masked language modeling (MLM) to pretrain on both static and dynamic traces collected by micro-executing pieces of the program.
% The learned program representations of the pretrained model can then be used to boost the performance across many downstream tasks including precise and efficient binary similarity and platform-agnostic binary vulnerability search. These capabilities are essential, especially given the popularity of today's IoT devices and broad deployment of firmware images.

Semantic function similarity, which quantifies the behavioral similarity between two functions, is a fundamental program analysis capability with a broad spectrum of real-world security usages, such as vulnerability detection~\cite{brumley2008automatic}, exploit generation~\cite{avgerinos2014automatic}, tracing malware lineage~\cite{jang2013towards, bayer2009scalable}, and forensics~\cite{luo2014semantics}.
% An effective binary clone search engine can substantially reduce the manual effort in reverse engineering, especially when analyzing stripped binaries such as commercial-off-the-shelf programs, legacy programs, and malware.
% It has a broad spectrum of real-world security usages, such as vulnerability detection~\cite{brumley2008automatic}, exploit generation~\cite{avgerinos2014automatic}, tracing malware lineage~\cite{jang2013towards, bayer2009scalable}, and forensics~\cite{luo2014semantics}.
For example, OWASP lists ``using components with known vulnerabilities'' as one of the top-10 application security risks in 2020~\cite{OWASP}.
Therefore, identifying similar vulnerable functions in massive software projects can save significant manual effort.

When matching semantically similar functions for security-critical applications (\eg vulnerability discovery), we often have to deal with software at \emph{binary level}, such as commercial off-the-shelf products (\ie firmware images) and legacy programs.
However, this task is challenging as the functions' high-level information (\ie data structure definitions) are removed during the compilation process. 
The problem aggravates when the functions are compiled to run on different instruction set architectures with various compiler optimizations or even simple obfuscations.
% as the same high-level functionality can be implemented in dramatically different code~\cite{kamiya2002ccfinder, jiang2007deckard, gabel2008scalable}.
% The problem aggravates at the binary level because of two reasons. 
% First, 
% Second, the compiled functions can run on different instruction set architectures and compiled by various optimizations or obfuscations.
% The problem aggravates when the functions are compared at the binary level, where their high-level information (\ie variable names, comments, and data structure definitions) are often absent due to compilation.
% The compilation process further complicates the task by producing function binaries running on different instruction set architectures and transforming the program logic with various optimizations or even obfuscations, resulting in entirely different binary code syntax.
% compiled to different instruction set architectures, resulting in entirely different binary syntax.
% Various settings in the compilation process, such as optimizations or even obfuscations, further complicate the task.

There has been a growing interest in using Machine Learning (ML) to tackle these challenges~\cite{xu2017neural, massarelli2019safe, ding2019asm2vec}.
Notably, ML models learn function representations (\ie embeddings) from instructions in function binaries and match the functions based on the learned representation.
These approaches have obtained the state-of-the-art results~\cite{xu2017neural, massarelli2019safe, ding2019asm2vec}, outperforming the traditional signature-based approaches~\cite{bindiff} that rely on the hand-coded features (\eg number of basic blocks) extracted by domain experts. 
% Traditional approaches match two functions based on their features that encode the function's syntactic and structural characteristics extracted by human experts~\cite{bindiff, egele2014blanket, ming2017binsim}. 
% For example, BinDiff~\cite{bindiff}, the commercial binary comparison tool, extracts the function name, the number of basic blocks, and the number of function calls to determine the similarity.
% In addition to the static approach, dynamic approaches (\eg iLine~\cite{jang2013towards}, Blex~\cite{egele2014blanket}, BinSim~\cite{ming2017binsim}) selects the dynamic features by executing the function, such as values read/written from/to program stack/heap~\cite{egele2014blanket} or system calls~\cite{ming2017binsim}.
% However, hand-crafted features are often \emph{incomplete} to encode function semantics~\cite{mckee2019software}, resulting in sub-optimal accuracy when two function binaries have tremendously different syntax or structures.
% Moreover, collecting some features (\eg neighbors in the call graph~\cite{bindiff}) and the comparison algorithms (\eg graph matching~\cite{bindiff} and symbolic execution~\cite{ming2017binsim}) are expensive, which significantly limits their \emph{scalability}.
% There has been a growing interest using Machine Learning (ML) to address these challenges.
% Notably, learning a distributed representation, \ie an embedding, of a function has obtained the state-of-the-art results~\cite{xu2017neural, massarelli2019safe, ding2019asm2vec} for matching function binaries. 
% As empirically demonstrated, the learned embedding encodes function semantics more closely than the hand-crafted features~\cite{massarelli2019investigating}.
The ML-based approaches are also amenable to large-scale function matching as computing similarity score as embedding distance is exceptionally efficient (\eg taking around 0.1 seconds searching over one million functions)~\cite{feng2016scalable}.
% Specifically, the learned function embeddings are compared by a chosen similarity metric defined on the vector space (\eg cosine similarity).

% \subsection{Challenges}

\vspace{0.01cm}\noindent\textbf{Execution semantics.}
Despite the impressive progress, it remains challenging for these approaches to match semantically similar functions with disparate syntax and structure~\cite{mckee2019software}. 
An inherent cause is that the code semantics is characterized by \emph{its execution effects}. 
% Learning such execution semantics requires understanding .
However, all existing learning-based approaches are \emph{agnostic to program execution semantics}, taking the static code as the only input. 
Such a setting can easily lead a model into learning simple pattern matching, limiting their accuracy when such patterns are absent or changed~\cite{payer2014similarity, aghakhani2020malware}.

% For example, one of the popular modeling strategies~\cite{ding2019asm2vec, massarelli2019safe} is to treat binary code as a sequence tokens~\cite{massarelli2019safe} (\eg like a sentence in natural language).
% However, program code's semantics is based on the understanding of how it executes.
Take a pair of x86 instructions as an example. \texttt{mov eax,2;lea ecx,[eax+4]} are semantically equivalent to \texttt{mov eax,2;lea ecx,[eax+eax*2]}.
To determine their similarity statically, the most salient pattern is their common substring (both sequences share the tokens \texttt{mov}, \texttt{eax}, \texttt{lea}, \texttt{ecx}), which does not encode the key reason of equivalence.
% learning spurious correlation that, \eg common tokens imply the similarity (both sequences share the tokens \texttt{mov}, \texttt{eax}, \texttt{lea}, \texttt{ecx}).
Without grasping the execution semantics, an ML model can easily learn such spurious patterns without understanding the inherent cause of the equivalence: \texttt{[eax+eax*2]} computes the same exact address as \texttt{[eax+4]} when \texttt{eax} is 2.
% The ML model cannot understand the inherent equivalence is due to the fact that the address of \texttt{[eax+eax*2]} equals to that of \texttt{[eax+4]} when \texttt{eax} is 2.
% This is because the static assembly code does not reveal the execution semantics of instruction (\eg \texttt{mov}, \texttt{lea}, and the arithmetic operations) to the model. 
% Therefore, the model does not know \texttt{mov} assigns \texttt{eax} to 2. Nor does the model understand \texttt{lea} loads the effective address of \texttt{[eax+4]} and \texttt{[eax+eax*2]}, which are both essentially equal to 6.

% For a same source function compiled to two function binaries with different syntax, their execution semantics preserves the fundamental invariance resilient to syntactic changes, critical to determining whether they are similar.
% Therefore, to teach an ML model with the execution semantics, the model should observe a function's dynamic behavior during training.
% However, static information is inadequate in exposing such knowledge.

\vspace{0.01cm}\noindent\textbf{Limitations of existing dynamic approaches.}
Conceptually, dynamic analysis captures the perfect execution semantics.
However, traditional dynamic analysis is inappropriate here as it is hard to find a concrete program input exercising a certain function of interest.
While symbolic execution can help, it is known for poor scalability to large programs.

Therefore, existing dynamic approaches~\cite{egele2014blanket} \emph{relax} the function initial states with random values that are often under-constrained -- they may not be feasible from executing the program regularly.
For example, a function \texttt{bar()} can only be executed when called by function \texttt{foo()}.
When directly executing \texttt{bar()}, the constraints of \texttt{bar()}'s initial states imposed in \texttt{foo()} is ignored.
While these approaches can directly execute individual functions and compare their execution behavior, such a relaxation introduces \emph{noisy and incomplete traces}.
% (despite getting outperformed by the ML-based approaches based only on static code~\cite{ding2019asm2vec})
% Learning execution semantics requires collecting execution traces as training data.
% % However, implementing such a tracing tool for individual functions is challenging in practice.
% Traditional dynamic analysis is inappropriate as it is hard to find a concrete program input exercising a certain function of interest.
% While symbolic execution can help, it is known for poor scalability to large programs.
% They can thus execute individual functions without executing the whole program from the beginning.
% While their approaches make use of execution semantics to compute similarity, they assume the function can take arbitrary values and obtain execution behavior by randomly-sampled function inputs.
% However, to obtain individual function's execution behavior, these approaches \emph{sample random function inputs} to directly emulate the function without executing the whole program from beginning.
% While this can mitigate the problem of low coverage in traditional dynamic analysis (as it is hard to find a concrete program input exercising a certain function of interest), 
% However, such a relaxation introduces \emph{noisy and incomplete traces}.
% Besides, the randomly generated inputs can also fail to trigger complete function behavior.
For example, for functions taking only values from specified range, \eg $\sqrt{x}$ and $arcsin(x)$, the randomized function inputs (\eg negative numbers for $\sqrt{x}$ and numbers outside $[-1,1]$ for $arcsin(x)$) often trigger the similar behavior such as the exception handling.
Therefore, existing dynamic approaches suffer from false positives~\cite{ding2019asm2vec}.


% Moreover, similar to traditional approaches, existing dynamic approaches also resort to hand-coded (dynamic) features to match functions, which can be incomplete in exposing function behavior. 
% For example, none of the 7 dynamic features (\ie values stored/read to/from stack/heap) defined in Blex can detect whether two arithmetic instructions (\eg \texttt{xor eax,eax} and \texttt{mov eax,0}) have the same execution effect as they do not access the memory (see Section~\ref{sec:overview} for details).

% the randomly initialized function arguments is likely never feasible when executing the program normally.

% To match functions' dynamic behavior, existing approaches still resort to signature-based matching by extracting manually-defined features.
% For example, Blex defines 7 features (\eg values read/write to/from program memory) that summarize the execution side effect from the potentially imprecise function execution.
% These features are thought to encode partial execution semantics, useful to determining function similarity.
% The rationale of such relaxation is that partial execution semantics is still preserved from the noisy traces.

% More importantly, the hand-crafted features can be \emph{brittle to noises introduced by the relaxed execution semantics}. 
% For instance, for functions only called with specific arguments, the randomized argument values can often trigger the similar behavior (in terms of the feature values) such as the exception handling, leading to false positives.


\vspace{0.01cm}\noindent\textbf{Our approach.}
This paper presents \sys (\emph{TRansfer-learning EXecution semantics}) that matches semantically similar functions based on their static instructions but augmented with execution semantics.
Instead of using noisy and incomplete dynamic trace to directly determine similarity, \sys first pretrains the model to observe and understand how each instruction executes in a function.
% As shown in Figure~\ref{fig:general}, it first pretrains the model to observe and understand how each instruction executes in a function, instead of using noisy functions' behavior to directly determine similarity.
It then \emph{transfers} and \emph{composes} the learned knowledge from pretrained model to match semantically similar functions.
% The pretraining task is unsupervised and automated, which does not need any effort of manual labeling and feature engineering.
% To obtain the dynamic behavior, we implement micro-execution~\cite{godefroid2014micro} to \emph{micro-trace} functions across multiple architectures without the need to execute the whole program from the beginning.
% We develop a hierarchical Transformer~\cite{vaswani2017attention} architecture to efficiently encode the execution semantics as embeddings from raw assembly instructions and micro-traces.
Our extensive experiments suggest that the learned knowledge of executions in pretraining significantly boosts the performance of matching semantically similar function binaries -- \sys excels in matching functions from different architectures, optimizations, and obfuscations.

% Unfortunately, existing tracing implementations for binary similarity only approximate the execution effect using \emph{coarse-grained} features summarized from the dynamic traces.
% For example, Blex~\cite{egele2014blanket} logs the values read/write from the program stack/heap to represent a function's dynamic behavior.
% These features cannot precisely describe the execution, leading to sub-optimal accuracy (Section~\ref{sec:eval}).

% Traditional dynamic analysis and symbolic execution are limited by low coverage (thus may not even reach the target function) and poor scalability to large programs.

% For example, Blex~\cite{egele2014blanket, ming2017binsim} directly emulate executing functions based on a predefined policy (\eg randomly-initialized registers and function arguments).
% Unfortunately, their approaches summarize \emph{coarse-grained} features .

% Fine-grained binary tracing, however, is \emph{computationally demanding}.
% For example, to closely emulate a program's actual execution, X-Force~\cite{peng2014x} spends substantial engineering effort such as inferring indirect jump targets and handling library function calls.
% This limits their practicability as binary clone search often operates on the orders of hundred millions of functions~\cite{feng2016scalable}. 

% Ours simplified micro-tracing design, potentially noisy traces but (1) expose diverse behavior (2) our model is resilient to moderate noises in learning instruction-level execution semantics.

% \kexin{Some papers use dynamic analysis, but they are restricted by coarse-grained manual feature selection (blanket execution: 7 features, binsim: only system/API calls slices) and poor scalability (binsim: dynamic slicing and symbolic execution).}

% \kexin{These limitations have been briefly described in 3rd/4th paragraphs since they do not use ML. Should we discuss them here? as the reader may wonder ``No, there are dynamic approaches'' when reading up to here (although I have emphasized ``ML approaches are the SOTA 
% but none of ML approaches used execution''.)}

% \kexin{Might remove - trivial and too ML.. I just dumped here in case they can be used somewhere}
% Besides the absence of dynamic information, all existing approaches are fundamentally limited by their ML architecture and task design, facing the following challenges.

% \vspace{0.01cm}\noindent\textbf{Context.}
% To learn function embeddings from a potentially long execution trace, the ML architecture should be able to model \emph{long-range execution effect} (\eg dataflow dependencies within a long execution trace)~\cite{khandelwal2018sharp}.
% However, the ML architectures used in all previous works encode only \emph{localized context}~\cite{ding2019asm2vec, duandeepbindiff}.
% For example, Asm2Vec~\cite{ding2019asm2vec} extends the Word2Vec PV-DM algorithm by setting context window size to 3 -- the instructions that are not neighbors of the current instruction are not included in the computation of its embedding.

% The challenge of learning long-range dependencies is partly addressed by encoding program structures, \eg control flow graph, in a graph neural network~\cite{xu2017neural}, where its message-passing mechanism can propagate information to distant nodes.
% However, their graph construction is expensive (\eg taking up to $1000$ seconds for large functions).
% Moreover, the challenge of using only coarse-grained features remains -- only 7 summarized features (\eg number of instructions) are extracted for each graph node based on heuristics.

% For example, to learn an effective representation of the function parameter (useful to determine the function similarity), the model has to encode how the function parameters are accessed within the function.
% However, instructions that operate on the function parameter can be far away from the instruction that initialize the parameter.

% The learned embeddings from all existing works encode \emph{only limited context}, inefficient in modeling long-range dependencies in the execution traces.
% For example, they either extend Word2Vec~\cite{mikolov2013distributed} or leverage graph neural network to learn code embeddings from their context.
% Both models suffer from restricted context size.
% For example, DeepBinDiff~\cite{duandeepbindiff} extends Word2Vec CBOW algorithm by using only 3 as the context window size. 
% Gemini~\cite{xu2017neural} uses 5-hop message-passing propagation among the node neighbors within the control flow graph. 
% Increasing the context size in these models, however, incurs significant runtime and memory overhead. For example, the number of hops in the graph neural network determines the number of layers in the graph neural network (\ie number of iterations for message passing)

% \vspace{0.01cm}\noindent\textbf{Structured knowledge.}
% Either do not encode structured knowledge (Word2Vec/RNN), or too expensive (GNN).
% Function structure (\eg control flow) provides critical hint on a function's logic.
% Encoding such structured knowledge as an inductive bias in the model has been shown improving the model's generalizability and data-efficiency~\cite{xu2017neural,duandeepbindiff}.

% However, existing approaches:
% Encoding to graph - large graph hard to scale, manual effort for feature extraction.
% Encoding to sequence, word2vec model, RNN model. Assume sequential dependencies.

% \subsection{Our Approach}

% Our results on 423,349,054 binary functions show that \sys outperforms all state-of-the-art tools in accuracy at searching over functions, and is robust to changes brought by different instruction architectures, compiler optimizations, and obfuscations. 
% Additionally, \sys's speed is on par with the fastest tools.

\begin{figure*}[!t]
\centering
\includegraphics[width=\linewidth]{./figs/general.pdf}

\caption{
The workflow of \sys. We first pretrain the model on the function code and its micro-traces (\ie dynamic register values) using the masked LM task. 
We then finetune the pretrained model on the function pairs (\eg same source function compiled to different architectures with different optimizations/obfuscations) by stacking new neural network layers for function similarity tasks. 
Finetuning updates both the pretrained model and the stacked layers. 
During inference, the finetuned model computes the function embedding, whose distance encodes the function similarity.}

\label{fig:general}
\end{figure*}

% Our key insight is to first teach the model with execution semantics, and then \emph{transfer} the learned knowledge to binary similarity task.
Our key insight is that the function's behavior can be \emph{composed} by each instruction's execution semantics, which can be learned by observing and understanding how each instruction executes in the dynamic traces.
For example, given instructions \texttt{mov eax,2;sub eax,1;add eax,3} and their dynamic traces, we can train the model to predict the value of \texttt{eax} after executing these instructions.
This training objective is designed to force the model to understand the execution semantics of \texttt{mov}, \texttt{sub}, and \texttt{add}, \ie how they manipulate the operands and updates the results, and learn to \emph{compose their execution effects} to understand their overall behavior.

We can then \emph{transfer} the model's learned knowledge to compose instructions' execution semantics to match semantically similar functions.
As a result, our approach is not constrained by noisy and incomplete traces -- it matches functions based \emph{only} on their \emph{complete} static instructions but \emph{augmented} with rich knowledge of execution semantics.
Such a design also saves significant runtime overhead as we do not need to execute any function on-the-fly when matching them~\cite{kapravelos2013revolver}.
% For example, by observing the value of \texttt{eax} before and after \texttt{add eax,num} and \texttt{sub eax,num} from many training samples with different \texttt{num}, the model can learn the actual execution semantics of \texttt{add} and \texttt{sub}, which helps the model to understand the inherent equivalence of \texttt{add ebx,1} and \texttt{sub ebx,-1}.
% Also, we leverage
% Our key insight is that model can learn to \emph{compose} its learned execution semantics of each static 

% Training \sys has two phases, as shown in Figure~\ref{fig:general}.
% The first phase \emph{pretrains} the model on both the function's assembly instructions and its micro-traces using masked Language Modeling (masked LM) to teach it execution semantics of diverse instructions.
% The second phase \emph{finetunes} the pretrained model on function pairs to match similar functions across different architectures, optimizations, and obfuscations.
% It takes as input the function and outputs its embedding.
% This new model is finetuned on function pairs such that the distance between its output embeddings encode the function similarity. 

% \vspace{0.01cm}\noindent\textbf{Learning execution semantics by pretraining.}
% The masked LM task is unsupervised and automated, which does not need any effort of manual labeling and feature engineering.
Given a sequence of assembly instructions and their micro-traces (\ie register values), we pretrain the model with the masked language modeling (masked LM) task.
Notably, it masks random parts in the sequence and asks the model to predict masked parts based on their context. 
This design forces the model to learn how a function executes to correctly infer the missing values. 
% \eg by observing how instructions manipulate the registers and memory , which \emph{automates} learning execution semantics instead of manually extracting features (see intuitive examples in Section~\ref{subsec:overview_pretrain}).
It thus \emph{automates} learning execution semantics without any manual feature engineering.
% the learned knowledge assists in understanding that the inherent similarity between syntactically-different functions is rooted in their similar execution behaviors, rather than the static patterns.
It also enables learning more \emph{comprehensive} execution semantics of diverse instructions, as we can mask various parts of the function, imposing the model to learn different aspects of execution semantics to make correct prediction.
Moreover, this task is fully \emph{unsupervised}.
Therefore, \sys can be trained and further improved using arbitrary binaries found in the wild.

% We give some intuition on why the masked LM task helps to learn execution semantics.
% Consider a sequence of instructions in a function \texttt{mov ecx,1; add ecx,3; push ecx; mov ebx,ecx; push ebx}.
% We mask the 4th \texttt{ecx} by replacing it with \texttt{<MASK>} and feed the resulting sequence to the model.
% To correctly predict \texttt{<MASK>}, which consists of both the name \texttt{ecx} and its dynamic value 4, the model has likely learned the following.
% (1) It should learn \texttt{mov} assigns \texttt{ecx} with 1 in the first instruction by observing that the dynamic value of \texttt{ecx} in \texttt{add ecx,3} is 1 (before executing the instruction).
% (2) It learns \texttt{add} performs addition that updates \texttt{ecx} to 4, by observing the value of \texttt{ecx} in \texttt{push ecx}.
% (3) It learns that \texttt{<MASK>} equals to 4, by observing the dynamic value of \texttt{ebx} in \texttt{push ebx} and applying its learned knowledge of \texttt{mov}.
% (4) It predicts that \texttt{<MASK>} has the dynamic value 4 with register name \texttt{ecx}.

% Note that masked LM also indirectly compels the model to learn implicit syntactic idiom of the binary code.
% For example, the training data should teach the model that \texttt{mov ebx,ebx} is unusual, thus leading the model to rank \texttt{ecx} much higher than \texttt{ebx} in the prediction of \texttt{<MASK>}.

% While it is trivial to simply memorize individual cases to predict \texttt{<MASK>}, the model maintaining high testing accuracy when pretrained on diverse functions strongly indicates it understands execution semantics of different instructions so it can generalize to accurately predict unseen dynamic values~\cite{wallace2019nlp}.

% \vspace{0.01cm}\noindent\textbf{Finetuning without noisy traces.}
% After pretraining, we finetune the model by feeding \emph{only the static assembly instructions without micro-traces}. 
% Our insight is that the pretraining task has endowed execution semantics to each opcode and operand so that the model during finetuning can leverage such knowledge to match functions.
% In contrast, all existing learning-based approaches always learn function matching from scratch so the trained model tends to take the shortcut by matching superficial patterns~\cite{geirhos2018imagenet}.
% As a result, the function matching in our setting is not constrained by incomplete or noisy dynamic traces -- it still uses the complete static instructions, but they are augmented with rich knowledge of execution semantics.
% Moreover, this setting saves significant runtime overhead as we do not need to execute each function on-the-fly when matching each function pair.

To encode both the static and dynamic information as the model inputs, we design a hierarchical Transformer~\cite{vaswani2017attention} that supports modeling concrete micro-trace values. 
By contrast, existing approaches often treat the numerical values as a dummy token~\cite{massarelli2019safe, ding2019asm2vec} to avoid prohibitively large vocabulary size, which cannot effectively learn the rich dependencies between concrete values that likely encode key function semantics.
Moreover, our architecture's self-attention layer is designed to model long-range dependencies in a sequence~\cite{vaswani2017attention} efficiently.
Therefore, \sys can support roughly 170$\times$ longer sequence and runs 8$\times$ faster than existing neural architectures, essential to learning embeddings of long function execution traces.
% Also, such setting enables efficient large-scale function searching, as we \emph{do not need to execute each function to compare the similarity} -- we perform micro-execution only during pretraining.
% This is a one-time effort~\cite{devlin2018bert, liu2019roberta} as opposed to all existing approaches based on dynamic analysis~\cite{egele2014blanket, ming2017binsim, mckee2019software}, which requires executing the function each time during comparison. 

% \vspace{0.01cm}\noindent\textbf{New models for learning traces.}
% Besides, we introduce several auxiliary input embeddings to encode spatial structures of function instructions into the model architecture (see Figure~\ref{fig:arch} detailed in Section~\ref{sec:method}).

% One of the key advantages of the Transformer (over other embedding networks) is that its self-attention layer is designed to efficiently model long-range dependencies in a sequence.
% Therefore, \sys can support roughly 170$\times$ longer sequence than existing approaches (\eg those based on Word2Vec~\cite{ding2019asm2vec, duandeepbindiff}), essential to learning embeddings of long function execution traces.

% \vspace{0.01cm}\noindent\textbf{Results.}
We evaluate \sys on 1,472,066 functions collected from 13 popular open-source software projects across 4 architectures (x86, x64, ARM, and MIPS) and compiled with 4 optimizations (\texttt{O0}-\texttt{O3}), and 5 obfuscation strategies~\cite{hikari}. 
\sys outperforms the state-of-the-art systems by 7.8\%, 7.2\%, and 14.3\% in matching functions across different architectures, optimizations, and obfuscations, respectively. 
Our ablation studies show that the pretraining task significantly improves the accuracy of matching semantically similar functions (by 15.7\%).
We also apply \sys in searching vulnerable functions in 180 real-world firmware images developed by well-known vendors and deployed in diverse embedded systems, including WLAN routers, smart cameras, and solar panels.
Our case study shows that \sys assists in finding 16 real-world CVEs in these firmware images, which have not been disclosed in any previous studies.
% ~\bray{It is not clear at all what applications did you study?}
% Furthermore, \sys's underlying neural architecture is highly parallelizable and efficient, running up to 38$\times$ faster than hand-written disassemblers like IDA Pro.
We make the following contributions.

\begin{itemize}
    \item We propose a new approach to matching semantically similar functions: we first train the model to learn program execution semantics and then transfer the learned knowledge to match semantically similar functions.
    
    % \item We demonstrate that masked LM is an effective task to automate learning execution semantics. We then show how this knowledge can be transferred to accurately match semantically similar functions across different architectures, compilers, optimizations, and obfuscations.
    
    \item We implement micro-execution to collect dynamic traces on different architectures. We then develop a novel neural architecture -- hierarchical Transformer -- that can efficiently learn execution semantics from micro-traces.

    \item We implement \sys and evaluate it on 1,472,066 functions from 13 popular software projects and libraries. \sys outperforms the state-of-the-art tools by 7.8\%, 7\%, and 14.3\%, in cross-architecture, optimization, and obfuscation function matching, respectively, while running up to 8$\times$ faster.
    % Ablation studies demonstrate that our pretraining with micro-traces can improve the function matching results by 15.7\%.
    Moreover, \sys helps uncover 16 vulnerabilities in 180 real-world firmware images with latest version that are not disclosed by previous studies.
    We release \sys at \url{anonymous.4open.science/r/644f4ceb-ab22-4f04-a91c-0565e091ca31}.

\end{itemize}
